Rethinking deep active learning: Using unlabeled data at model training

Active learning typically focuses on training a model on few labeled examples alone, while unlabeled ones are only used for acquisition. In this work we depart from this setting by using both labeled and unlabeled data during model training across active learning cycles. We do so by using unsupervised feature learning at the beginning of the active learning pipeline and semi-supervised learning at every active learning cycle, on all available data. The former has not been investigated before in active learning, while the study of latter in the context of deep learning is scarce and recent findings are not conclusive with respect to its benefit. Our idea is orthogonal to acquisition strategies by using more data, much like ensemble methods use more models. By systematically evaluating on a number of popular acquisition strategies and datasets, we find that the use of unlabeled data during model training brings a surprising accuracy improvement in image classification, compared to the differences between acquisition strategies. We thus explore smaller label budgets, even one label per class.

==> tex/overview.tex <==
\section{Overview}
\label{sec:overview}

\subsection{Discussed papers}
\begin{enumerate}
    \item\textbf{Large-scale visual active learning with deep probabilistic ensembles} \cite{chitta2018large} [11/2018]
    \begin{itemize}
        \item Standard approach to active learning. No pseudo-labels. Uses ensemble predictive entropy to choose samples for annotation.
        \item Uses core-set \cite{sener2018active} and ensemble \cite{beluch2018power} approaches as baselines. \textbf{Good paper to compare to.}
        \item DATASETS:  CIFAR-10, CIFAR-100, BDD100K and 5\% of IMAGENET
    \end{itemize}

    \item\textbf{Cost-effective active learning for deep image classification} \cite{wang2017cost} [12/2017]
    \begin{itemize}
        \item It introduces pseudo-labels in the context of deep active learning for high confidence samples. Based on a low enough entropy (under a given threshold). Combines this approach with 3 standard active learning strategies (entropy, margin, low probability).
        \item \textbf{Possible baseline} for semi-supervised approaches. Good paper overall.
        \item DATASETS:  Caltech-256, CACD
    \end{itemize}

    \item\textbf{Active learning for convolutional neural networks: A core-set approach} \cite{sener2018active} [02/2018]
    \begin{itemize}
        \item Core-set approach to active learning.
        \item Uses CEAL \cite{wang2017cost} as one of the baselines for semi-supervised experiments.
        \item DATASETS: CIFAR-10, CIFAR-100, Caltech-256, SVHN
    \end{itemize}


    \item\textbf{Deep bayesian active learning with image data} \cite{gal2017deep} [03/2017]
    \begin{itemize}
        \item Bayesian convolutional neural network.
        \item Using dropout during inference -- Monte Carlo dropout (MC-dropout).
        \item The model is used with different active learning approaches: entropy, BALD, mean STD, variation ratios and random.
        \item Compares favorably with \alert{semi-supervised} learning approaches.
        \item DATASETS: MNIST, ISIC 2016
    \end{itemize}


    \item\textbf{The power of ensembles for active learning in image classification} \cite{beluch2018power} [2018]
    \begin{itemize}
        \item MC-dropout, ensemble-based entropy (with respect to the weights) and geometric approaches (Core-set and REPR) evaluated. Ensemble approaches are the best.
        \item MC-dropout performs worse due to shared gradient and lower effective model capacity (some neurons are inactive).
        \item \textbf{Can we use the same baselines?}
        \item DATASETS: MNIST, CIFAR-10,  Diabetic Retinopathy, parts of IMAGENET
    \end{itemize}

    \item\textbf{Adversarial Sampling for Active Learning} \cite{mayer2018adversarial} [08/2018]
    \begin{itemize}
        \item GANs for active learning. First paper of this kind. Generates a candidate and matches with the closest existing sample for annotation.
        \item Better than random sampling in most cases. Worse than maximal entropy, but more efficient, supposedly.
        \item \textbf{Not that interesting for now.}
        \item DATASETS: MNIST, CIFAR-10
    \end{itemize}


\end{enumerate}

\subsection{New papers}
\begin{enumerate}
    \item\textbf{Deep active learning over the long tail} \cite{geifman2017deep} [11/2017]
    \begin{itemize}
        \item Based on the core-set approach (no citation of the other paper). Farthest first traversal. Chooses unlabeled points furthers from the already labeled.
        \item DATASETS: MNIST, CIFAR-10, CIFAR-100
    \end{itemize}

    \item\textbf{Deep active learning with a neural architecture search} \cite{geifman2018deep} [11/2018]
    \begin{itemize}
        \item Stacks Resnet blocks during the active learning process.
        \item Modular search space, adding stacks (group of blocks with the same width) or block of layers.
        \item Softmax response, MC-dropout and coreset as query functions.
        \item DATASETS: CIFAR-10, CIFAR-100, SVHN
    \end{itemize}

    \item\textbf{Learning active learning from data} \cite{NIPS2017_7010} [06/2017]
    \begin{itemize}
        \item Meta AL.
        \item Not used with deep learning (one sample at a time).
        \item DATASETS: CIFAR-10, CIFAR-100, SVHN
    \end{itemize}

    \item\textbf{Efficient active learning for image classification and segmentation using a sample selection and conditional generative adversarial network} \cite{mahapatra2018efficient} [06/2018]
    \begin{itemize}
        \item A conditional GAN approach.
        \item Generate images which are added to the labeled set based on the informativeness provided by Bayesian neural network.
        \item DATASETS: SCR chest XRay
    \end{itemize}

     \item\textbf{QBDC: Query by dropout committee for training deep supervised architecture} \cite{ducoffe2015qbdc} [11/2015]
    \begin{itemize}
        \item Query by committee for deep neural networks.
        \item Batchwise dropout.
        \item DATASETS: MNIST
    \end{itemize}

    \item\textbf{Discriminative active learning} \cite{anonymous2019discriminative} [2019?]
    \begin{itemize}
        \item Good code for evaluation (implemented baselines).
        \item Tries to make the labeled and unlabeled set indistinguishable. AL as a binary classification task. Selects samples that are mostly likely to belong to the unlabeled set.
        \item Still under review for ICLR 2019: \url{https://openreview.net/f   orum?id=rJl-HsR9KX}
        \item DATASETS: MNIST, CIFAR-10
    \end{itemize}

    \item\textbf{Adversarial active learning for deep networks: a margin based approach} \cite{ducoffe2018adversarial} [2/2018]
    \begin{itemize}
        \item Selects the samples based on adverserial examples (Deep-Fool). Samples with the lowest norm perturbation are selected. Both the sample and its adversary are added to the labeled set.
        \item Compares to CEAL \cite{wang2017cost} and CORE-SET \cite{sener2018active} among others.
        \item DATASETS: MNIST, Shoe-Bag, Quick-Draw
    \end{itemize}


\end{enumerate}

